Learning to Remember from a Multi-Task Teacher

Recent studies on catastrophic forgetting during sequential learning typically focus on fixing the accuracy of the predictions for a previously learned task. In this paper we argue that the outputs of neural networks are subject to rapid changes when learning a new data distribution, and networks that appear to "forget" everything still contain useful representation towards previous tasks. Instead of enforcing the output accuracy to stay the same, we propose to reduce the effect of catastrophic forgetting on the representation level, as the output layer can be quickly recovered later with a small number of examples. Towards this goal, we propose an experimental setup that measures the amount of representational forgetting, and develop a novel meta-learning algorithm to overcome this issue. The proposed meta-learner produces weight updates of a sequential learning network, mimicking a multi-task teacher network's representation. We show that our meta-learner can improve its learned representations on new tasks, while maintaining a good representation for old tasks.

==> sections/acknowledgment.tex <==
% !TEX root = ../main.tex
\paragraph{Acknowledgment} We would like to thank Pumpki Lei Su for helpful discussion and
providing references to related literature in language acquisition.

==> sections/exp2fig.tex <==
% !TEX root = ../main.tex
% \begin{figure}[t]
% \vspace{-0.2in}
% \begin{center}
% \begin{minipage}{0.47\linewidth}
% \begin{figure}[H]
% \vspace{-0.1in}
% \includegraphics[width=1.0\linewidth, trim={0cm 0cm 0cm 0cm},clip]{figures/cifar100_acc_iclr_new.pdf}
% \vspace{-0.2in}
% \caption{\small Experiment 2: Unseen classes}
% \label{fig:cifar100}
% \end{figure}
% \end{minipage}
% % \hfill
% \quad
% \quad
% \begin{minipage}{0.47\linewidth}
% \begin{figure}[H]
% \vspace{-0.1in}
% \centering
% \includegraphics[width=1.0\linewidth]{figures/cifar100_multi_snapshot_acc_iclr_new.pdf}
% \vspace{-0.2in}
% \caption{\small Experiment 3: Unseen initialization}
% \label{fig:cifar100_multisnap}
% \end{figure}
% \end{minipage}
% \end{center}
% \vspace{-0.1in}
% \end{figure}

\begin{figure}[t]
\begin{center}
% \includegraphics[width=0.48\linewidth, trim={0cm 0cm 0cm 0cm},clip]{figures/cifar100_acc_iclr_new.pdf}
\includegraphics[width=\linewidth]{figures/cifar100_acc_icml.pdf}
\vspace{-0.2in}
\caption{
%\textbf{Left:} 
%Exp 3: CIFAR 5A $\mapsto$ 100 with unseen initialization checkpoints. ``Freeze'' has 92.25\% on Task A and 71.68\% on Task B. Error bar denotes standard error of the mean of 5 runs.
 Exp 2: CIFAR 5A $\mapsto$ 100 with unseen classes; 
%\textbf{Right:} Tiny-ImageNet \mengye{finish this}
}
\label{fig:exp2}
\end{center}
\vspace{-0.1in}
\end{figure}

==> sections/filterfig.tex <==
% !TEX root = ../main.tex
\begin{figure}[t]
\vspace{-0.3cm}
\centering
\begin{tabular}{ccc}
\includegraphics[width=0.25\textwidth]{figures/baseline_400.pdf} &
\includegraphics[width=0.25\textwidth]{figures/teacher_400.pdf} &
\includegraphics[width=0.25\textwidth]{figures/ours_400.pdf}\\
(a) baseline & (b) multi-task teacher & (c) meta-learner
\end{tabular}
\vspace{-0.1cm}
\caption{MNIST $\mapsto$ FashionMNIST: Changes in the first layer weights after 400 update steps}
\label{fig:meta}
\end{figure}

==> sections/metafig.tex <==
% !TEX root = ../main.tex
\begin{figure*}[t]
% \vspace{-0.2in}
\centering
% \fbox{
\includegraphics[width=0.7\textwidth,trim={0cm 13.4cm 15.5cm 0cm},clip]{figures/metamodule.pdf}
\vspace{-0.15in}
% }
\caption{Our meta-learner module is a stacked LSTM network. For a given output neuron $h'_j$, the
meta-network takes in its activation, its pre-activations, current weights and gradients, and output
the weight updates assiciated with $h'_j$. Weights in the same layer will be shared a single
meta-network,  while different layers will have different nmeta-networks.}
\label{fig:meta}
% \vspace{-0.3in}
\end{figure*}

==> sections/tab_all.tex <==
% !TEX root = ../main.tex

% ICLR 2020
% \begin{table*}[t]
% % \vspace{-0.5in}
% \begin{center}
% \begin{small}
% % \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{ccccc}
% \toprule
%                  & Exp 1 MNIST/Fashion  & Exp 1 CIFAR-5A/5B   & Exp 2 CIFAR-5A/100  & Exp 3 CIFAR-5A/100  \\
% \midrule
% Freeze           & 84.8                 & 65.1                & 68.6 $\pm$ 2.9      & 68.6 $\pm$ 2.9      \\ 
% \midrule
% SGD              & 86.8 $\pm$ 1.0       & 68.7 $\pm$ 1.5      & 71.0 $\pm$ 2.1      & 71.0 $\pm$ 2.1      \\
% SGD $\times$ 0.1 & 85.0 $\pm$ 0.7       & 65.4 $\pm$ 2.1      & 69.7 $\pm$ 2.3      & 69.7 $\pm$ 2.3      \\
% LwF              & 87.2 $\pm$ 1.1       & 69.3 $\pm$ 0.7      & 73.1 $\pm$ 1.7      & 73.1 $\pm$ 1.7      \\
% EWC              & 86.9 $\pm$ 1.7       & 67.7 $\pm$ 1.0      & 72.9 $\pm$ 2.1      & 72.9 $\pm$ 2.1      \\
% Ours             & {\bf 87.3} $\pm$ 0.7 & {\bf 70.5} $\pm$ 1.1& {\bf 75.0} $\pm$ 1.3& {\bf 73.6} $\pm$ 2.6\\
% \midrule
% Teacher          & 88.0 $\pm$ 1.1       & 76.7 $\pm$ 0.3      & 81.9 $\pm$ 1.2      & 81.9 $\pm$ 1.2      \\
% \bottomrule
% \end{tabular}
% \end{small}
% % }
% % \vspace{0.2cm}
% \caption{Joint task performance on Experiment 1, 2 \& 3, after 500 update
% steps. $\pm$ denotes standard error of the mean of 5 runs.}
% \label{table:all}
% \vspace{-0.1in}
% \end{center}
% \end{table*}

% ICML 2020
\begin{table*}[t]
% \vspace{-0.5in}
\begin{center}
\begin{small}
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{ccccc}
\toprule
                 & Exp 1 CIFAR-5A/5B   & Exp 2 CIFAR-5A/100  & Exp 3 CIFAR-5A/100   & Exp 4 CFIAR-5A/tImgNet        \\
\midrule                                                                                                              
Freeze           & 65.1                & 68.6 $\pm$ 2.9      & 68.6 $\pm$ 2.9       &                               \\ 
\midrule                                                                                                                     
SGD              & 68.7 $\pm$ 1.5      & 71.0 $\pm$ 2.1      & 71.0 $\pm$ 2.1       &                               \\
SGD $\times$ 0.1 & 65.4 $\pm$ 2.1      & 69.7 $\pm$ 2.3      & 69.7 $\pm$ 2.3       &                               \\
LwF              & 69.3 $\pm$ 0.7      & 73.1 $\pm$ 1.7      & 73.1 $\pm$ 1.7       &                               \\
EWC              & 67.7 $\pm$ 1.0      & 72.9 $\pm$ 2.1      & 72.9 $\pm$ 2.1       &                               \\
Rep              & -      &   73.0 $\pm$ 3.5    &    73.0 $\pm$ 3.5    &                               \\
MAML              & -      &  74.8 $\pm$ 1.0     &   {\bf 74.8} $\pm$ 1.0     &                               \\
Ours             & {\bf 70.5} $\pm$ 1.1& {\bf 75.0} $\pm$ 1.3& {\bf 73.6} $\pm$ 2.6 &                               \\
\midrule                                                                                                             
Teacher          & 76.7 $\pm$ 0.3      & 81.9 $\pm$ 1.2      & 81.9 $\pm$ 1.2       &                               \\
\bottomrule
\end{tabular}
\end{small}
% }
% \vspace{0.2cm}
\caption{Joint task performance. $\pm$ denotes standard error of the mean of 5 runs.}
\label{table:all}
\vspace{-0.1in}
\end{center}
\end{table*}


% wo_grad 500: 87.3 +- 0.6, 86.3 +- 0.7 67.2 +- 2.4
% wo_weight 500: 86.7 +- 1.3 85.8 +- 0.6 68.9 +- 0.8
% ours 500: 88.1 +- 0.4 84.7 +- 0.8 70.5 +- 1.1


% cifar100 at 2050/500
% ours: 88.4 +- 1.5 86.1 +- 2.6 78.3 +- 1.3
% lwf: 82.3 +- 1.8 89.0 +- 3.1 70.0 +- 4.3
% ewc: 79.4 +- 2.6 88.8 +- 2.7 68.5 +- 4.1
% teacher: 91.4 +- 0.14 88.5 +- 2.9 82.5 +- 1.6
% sgd: 81.4 +- 2.0 88.8 +- 3.6 67.4 +- 2.6
% sgd 0.1: 85.2 +- 1.4 81.4 +- 5.4 68.0 +- 3.2


% cifar100 multisnapshot at 2000/500
% ours: 85.8 +- 1.6 81.8 +- 4.0 74.1 +- 2.2

% cifar 10 at 500
% teacher: 91.4 +- 0.5 86.6 +- 0.6 76.7 +- 0.3
% lwf: 87.1 +- 0.6 87.8 +- 0.9 69.3 +- 0.7
% ewc: 86.6 +- 0.2 87.5 +- 0.6 67.7 +- 1.0
% sgd: 86.4 +- 0.3 88.0 +- 0.9 68.7 +- 1.5
% sgd 0.1: 87.0 +- 1.3 80.1 +- 1.6 65.4 +- 2.1

% mnist 3600 at 500
% teacher: 97.7 +- 0.3 80.8 +- 1.0 88.0 +- 1.1


==> sections/tab_cifar.tex <==
%% !TEX root = ../main.tex
%
%\begin{table}
%\centering
%\begin{tabular}{c|cc|cc|cc}
%\toprule         
%   \multirow{2}*{} & \multicolumn{2}{c|}{100 iter}  & \multicolumn{2}{c|}{200 iter} & \multicolumn{2}{c}{300 iter}\\
%                 & Task A  & Task B &  Task A & Task B & Task A & Task B    \\
%\midrule
%Freeze           & 92.632      &     69.804   &         \\ 
%\midrule
%SGD              & $85.96 \pm 1.56$ &  $79.984 \pm 0.33$  & $84.78 \pm 1.22$ & $83.74 \pm 0.77$ & $84.89 \pm 0.71$ & $85.57 \pm 0.48$       \\  
%SGD $\times$ 0.1 & $85.68 \pm 2.17$ &  $67.972 \pm 2.33$  & $85.78 \pm 1.76$ & $71.74 \pm 2.11$& $86.06 \pm 1.08$ & $75.03 \pm 1.54$        \\  
%LwF              & $86.69 \pm 1.27$ &  $79.612 \pm 0.66$  & $85.85 \pm 0.78$ & $83.82 \pm 0.91$& $85.70 \pm 0.78$ & $85.50 \pm 0.67$        \\  
%EWC              & $86.29 \pm 1.39$ &  $79.648 \pm 0.62$  & $84.96 \pm 1.00$ & $83.80 \pm 0.91$& $84.96 \pm 0.62$ & $85.48 \pm 0.36$       \\  
%Ours             & $89.38 \pm 1.38$ &  $76.256 \pm 1.35$  & $88.86 \pm 1.09$ & $80.62 \pm 0.63$& $88.29 \pm 1.18$ & $82.46 \pm 0.72$        \\  
%\midrule
%Teacher          & $91.71 \pm 0.09$ &  $76.000 \pm 0.76$  & $91.64 \pm 0.14$ & $80.23 \pm 0.46$& $92.01 \pm 0.12$ & $82.77 \pm 0.51$        \\ 
%\bottomrule
%\end{tabular}
%\caption{CIFAR 5A $\mapsto$ 5B}
%\end{table}

% !TEX root = ../main.tex

\begin{table}[t]
\vspace{-0.4cm}
\centering
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{c|cc|cc|cc}
\toprule         
   \multirow{2}*{} & \multicolumn{2}{c|}{100 iter}  & \multicolumn{2}{c|}{200 iter} & \multicolumn{2}{c}{300 iter}\\
                 & Task A  & Task B &  Task A & Task B & Task A & Task B    \\
\midrule
Freeze           & 92.6   & 69.8  &  92.6  & 69.8  & 92.6  & 69.8           \\ 
\midrule
SGD              & 86.0 $\pm$ 1.6   &  {\bf 80.0} $\pm$ 0.3  & 84.8 $\pm$ 1.2 & 83.7 $\pm$ 0.8 & 84.9 $\pm$ 0.7 & {\bf 85.6} $\pm$ 0.5   \\  
SGD $\times$ 0.1 & 85.7 $\pm$ 2.2   &  68.0 $\pm$ 2.3  & 85.8 $\pm$ 1.8 & 71.7 $\pm$ 2.1 & 86.1 $\pm$ 1.1 & 75.0 $ \pm$ 1.5   \\  
LwF \cite{lwf}   & 86.7 $\pm$ 1.3   &  79.6 $\pm$ 0.7  & 85.9 $\pm$ 0.8 & 83.8 $\pm$ 0.9 & 85.7 $\pm$ 0.8 & 85.5 $\pm$ 0.7   \\  
EWC \cite{ewc}   & 86.3 $\pm$ 1.1  &  79.7 $\pm$ 0.9  & 86.0 $\pm$ 1.2 & {\bf 84.4} $\pm$ 0.5 & 85.5 $\pm$ 1.2 & 85.2 $\pm$ 0.8   \\  
Ours             & {\bf 89.4} $\pm$ 1.4 &  76.3 $\pm$ 1.4  & {\bf 88.9 $\pm$ 1.1} & 80.6 $\pm$ 0.6 & {\bf 88.3} $\pm$ 1.2 & 82.5 $\pm$ 0.7   \\  
\midrule
Teacher          & 91.7 $\pm$ 0.1 &  76.0 $\pm$ 0.8  & 91.6 $\pm$ 0.1 & 80.2 $\pm$ 0.5 & 92.0 $\pm$ 0.1 & 82.8 $\pm$ 0.5   \\ 
\bottomrule
\end{tabular}
}
\vspace{0.2cm}
\caption{Results on CIFAR-10, Task A: CIFAR-5A and Task B: CIFAR-5B}
\label{table:cifar10}
\vspace{-0.3in}
\end{table}


==> sections/tab_cifar_2.tex <==
% !TEX root = ../main.tex
\begin{table}[t]
\centering
\vspace{-0.15in}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{c|cc|cc|cc}
\toprule         
   \multirow{2}*{} & \multicolumn{2}{c|}{100 iter}  & \multicolumn{2}{c|}{500 iter} & \multicolumn{2}{c}{1000 iter}\\
                 & Task A  & Task B &  Task A & Task B & Task A & Task B    \\
\midrule
Freeze           & 92.4   & 63.2  & 92.4   & 63.2  & 92.4   & 63.2    \\ 
\midrule
SGD              & 80.7 $\pm$ 4.9 & {\bf 76.4} $\pm$ 7.5 & 78.5 $\pm$ 5.3 & 87.1 $\pm$ 3.4 & 77.1 $\pm$ 4.6 & 89.4 $\pm$ 2.8 \\  
SGD $\times$ 0.1 & 86.6 $\pm$ 1.0 & 62.8 $\pm$ 7.3 & 85.1 $\pm$ 1.6 & 76.4 $\pm$ 7.0 & 83.6 $\pm$ 2.2 & 82.8 $\pm$ 4.4  \\  
LwF \cite{lwf}   & 81.6 $\pm$ 6.3 & 75.3 $\pm$ 6.7 & 80.9 $\pm$ 4.7 & {\bf 87.2} $\pm$ 3.7 & 80.8 $\pm$ 4.0 & 89.2 $\pm$ 3.6 \\  
EWC \cite{ewc}   & 80.9 $\pm$ 5.1 & 75.4 $\pm$ 7.7 & 80.1 $\pm$ 3.8 & {\bf 87.2} $\pm$ 3.7 & 78.4 $\pm$ 4.3 & {\bf 89.8} $\pm$ 3.0  \\  
Ours             & {\bf 90.1} $\pm$ 0.5 & 73.5 $\pm$ 5.3 & {\bf 87.6} $\pm$ 1.5 & 85.0 $\pm$ 3.0 & {\bf 84.6} $\pm$ 1.7 & 85.6 $\pm$ 3.7  \\  
\midrule
Teacher          & 91.4 $\pm$ 0.5 & 76.6 $\pm$ 5.2 & 90.9 $\pm$ 0.4 & 87.4 $\pm$ 3.4 & 91.0 $\pm$ 0.2 & 89.0 $\pm$ 3.6   \\ 
\bottomrule
\end{tabular}
}
\vspace{0.2cm}
\caption{Results on CIFAR100, at meta-training time Task B is 5 classes randomly chosen from the first 50 classes, at meta-test time Task B is 5 classes randomly chosen from the last 50 classes}
\label{table:cifar100}
\vspace{-0.5cm}
% \vspace{-0.2in}
\end{table}



% Results on CIFAR100 with multi snapshot

